SkyTrakx: A Toolkit for Simulation and Verification of Unmanned Air-Traffic Management Systems (Extended Version)

The key concept for safe and efficient traffic management for Unmanned Aircraft Systems (UAS) is the notion of operation volume (OV). An OV is a 4-dimensional block of airspace and time, which can express an aircraft's intent, and can be used for planning, de-confliction, and traffic management. While there are several high-level simulators for UAS Traffic Management (UTM), we are lacking a framework for creating, manipulating, and reasoning about OVs for heterogeneous air vehicles. In this paper, we address this and present SkyTrakx -- a software toolkit for simulation and verification of UTM scenarios based on OVs. First, we illustrate a use case of SkyTrakx by presenting a specific air traffic coordination protocol. This protocol communicates OVs between participating aircraft and an airspace manager for traffic routing. We show how existing formal verification tools, Dafny and Dione, can assist in automatically checking key properties of the protocol. Second, we show how the OVs can be computed for heterogeneous air vehicles like quadcopters and fixed-wing aircraft using another verification technique, namely reachability analysis. Finally, we show that SkyTrakx can be used to simulate complex scenarios involving heterogeneous vehicles, for testing and performance evaluation in terms of workload and response delays analysis. Our experiments delineate the trade-off between performance and workload across different strategies for generating OVs.

==> sec-monitoring.tex <==
\begin{comment}

\section{Failures and Monitoring}
\label{sec:monitor}


\paragraph*{Failures in UTM}

% UTM paragraph on failures (copy-pasted from the report): Operators (RPICs if separate entity) are responsible for remaining within the bounds of their flight volume(s) and tracking the aircraft location during all phases of flight, while meeting required performance criteria for the operation performed. Operators monitor for vehicle non-conformance and on-board equipment failures or degradation (e.g., lost link, engine failure). For situations where corrections cannot be made, Operators are responsible for notifying affected airspace users as soon as practical and executing a predictable response. USSs can assist the Operator in providing tracking and conformance monitoring capabilities and notifying affected airspace users when an event occurs. For offnominal situations that pose sufficient risk to manned aircraft operations, and where actionable, timely FAA/ATC intervention is achievable, the Operator (through the USS) notifies the FAA and sends data required to manage the event via FIMS.19
% 19: Off-nominal situations that pose sufficient risk to manned aircraft operations are identified through USSintegrated risk assessment algorithms.

In UTM, aircraft operators are responsible on ensuring that they abide their volume contracts, or according to our notation, their \opervols.
When a failure causes the aircraft to violate its contract, it should notify the USS, which in turn have to notify affected users.
The USSs can help the operator to track the aircraft and plan a safe alternative volume contract to follow without affecting other aircraft~\cite{utm_conops}.

\paragraph{Failures in $\protocol$}
In our protocol, we handle violations of contracts similar to UTM. These violations can be caused by aggressive maneuvers an agent chooses to do as described in the previous section, or because of any kind of failures, such as software or hardware ones, that can occur to the agent. The agents themselves report their violations of contracts to the \AirMgr. In their reports, they send alternative, or \emph{recovery}, contracts that they are expected to follow after the violations. When the \AirMgr receives a violation report with the recovery contract $\mathtt{rec\_contr_i}$ from agent $i$, the \AirMgr replaces its saved contract $\mathtt{contr\_arr[i]}$ with $\mathtt{rec\_contr_i}$. Moreover, the \AirMgr notifies the agents with contracts in $\mathtt{contr\_arr}$ that intersect with $\mathtt{rec\_contr_i}$ to alert them of the potential collision danger.

\paragraph{Experimental Results and Analysis}
We implemented the violation detection and mitigation mechanism explained above in our framework.
We tested our monitoring implementation in \Corr scenarios with four and six drones.
We used the \Conse strategy to create \opervol.
From Table~\ref{table:comparison}, we can see that there are zero violations of the contract.
This ensures that the violations are not because of maneuvers chosen by the agents,
but because of failures simulation as we will discuss next.
This allows for a better comparison of the results under differ failure probabilities in Table~\ref{table:monitoring}.

In order to generate violations that mimic faults in the aircraft, we generate fake waypoints outside the contracts.
Whenever an agent reaches a waypoint in its path, we flip a biased coin with a \emph{head} probability of 0.4 or 0.9.
This head probability represents the failure probability. If the toss is a \emph{tail}, we provide it with the exact next waypoint $\mathit{next\_wp}$ in the path to follow. If it is a head we create a noisy version of $\mathit{next\_wp}$ by adding independent Gaussian noise with mean zero and standard deviation five to each of the three dimensions of $\mathit{next\_wp}$.
%
An agent $i \in \ID$ checks if its position and time is in its volume contract regularly. Whenever it recognizes it violated it, it generates its recovery contract $\mathtt{rec\_contr_i}$ using \inlinekrd{waypoints2contract} with arguments being its current position, current time, and the list of waypoints in the path that have not been visited yet. It sets $\mathtt{plan\_contr_i}$ and $\mathtt{curr\_contr_i}$ to $\mathtt{rec\_contr_i}$ and sends the latter to the \AirMgr to update $\mathtt{contr\_arr[i]}$ accordingly.
%

The results of our monitoring experiments are shown in Table~\ref{table:monitoring}.
In addition to the average response time per agent (Resp. T. (s)),
the number of rectangles per second in \Contracts which the \AirMgr has to check the disjointness of (\Rect/s),
and the violation rate (\Vio),
we report the number of alert notifications sent to agents per violation (\#notif./F).
We repeated each experiment five times and took the average of their results.


\begin{table}[t]
    \caption{Comparison of simulation time and agents notification rate between different fault probabilities and different numbers of agents.}\label{table:monitoring}

\begin{center}
    \begin{tabular}{|l|r|r|r|r|r|}
        \hline
        Failure Prob. & \Agt & Resp. T.(s) & \Rect/s &    \Vio & \#notif./F \\ \hline
        0.4           &    4 &       35.44 &    2.49 & 33.12\% &       0.43 \\
                      &    6 &       44.53 &    4.88 & 36.25\% &       0.42 \\ \hline
        0.9           &    4 &       54.73 &    1.56 & 74.38\% &       0.17 \\
                      &    6 &       54.81 &    4.44 & 72.92\% &       0.42 \\ \hline
    \end{tabular}
\end{center}

Failure Prob. is the probability to instrument waypoints outside of an agent's \contract,
\Agt is the number of agents,
Resp. T.(s) is the average response time per agent,
\Rect/s is the number of rectangles per second in \Contracts which the \AirMgr has to check the disjointness of,
\Vio is the violation rate,
and \#notif./F is the number of alert notifications sent to agents per violation.
\end{table}

As expected, the percentage of violations \Vio increases as the probability of failure increase. Moreover, the number \#notif./F seems independent of the number of drones and the number of failures. This is because the number of notifications sent depends on the number of surrounding agents that might be affected by an agent's violation of contract. If more air vehicles are added to a scenario, but the number of those that are close to each other remained the same, the number of notifications per violation would not be affected.
This is the case in the \Corr scenario, where there are at most two close air vehicles at any time independent of the total number of air vehicles.
Closeness of air vehicles in turn depends on the severity of the considered failures and the extent of contract violations before recovery. Such extent is determined in our experiments by the mean and the variance of the added Gaussian noise to the waypoints. Table~\ref{table:monitoring} uses the same Gaussian distribution to generate noise. We leave such comparison for future investigation.
With more number of violations, more checks have to be done by the \AirMgr to know which agents should be sent alerts. This is can be seen in Table~\ref{table:monitoring} by comparing the average response time Resp. T.(s) of the scenarios with failure probability 0.4 and those with 0.9. The latter are significantly larger than the former. Lastly, as the number of air vehicles increase, \Rect/s increases because of the increasing number of needed checks done by the airspace manager.

Finally, our framework allows also for violations monitoring by the airspace manager. This monitoring can be a similar, but centralized approach, of what the agents do of checking inclusion of their position-time pairs in their contracts. Or, it can be based on forecast to the future using simulation forward or reachability analysis to predict violations of contracts. % We keep these ideas for future investigation.








%\subsection{Basic}
%Under what conditions (physical speed of aircraft, and its environment, computation and sensing speed) can we check that the aircraft is going to violate its \contract.

%Current state is not in \contract---straightforward.

%\subsection{Advanced/predictive}

%We can raise an alarm $T_a$ time before a contract is violated?

\end{comment}

